Can Large-Language Models Help us Better Understand and Teach the Development of Energy-Efficient Software?

Computing systems are consuming an increasing and unsustainable fraction of society's energy footprint, notably in data centers. Meanwhile, energy-efficient software engineering techniques are often absent from undergraduate curricula. We propose to develop a learning module for energy-efficient software, suitable for incorporation into an undergraduate software engineering class. There is one major problem with such an endeavor: undergraduate curricula have limited space for mastering energy-related systems programming aspects. To address this problem, we propose to leverage the domain expertise afforded by large language models (LLMs). In our preliminary studies, we observe that LLMs can generate energy-efficient variations of basic linear algebra codes tailored to both ARM64 and AMD64 architectures, as well as unit tests and energy measurement harnesses. On toy examples suitable for classroom use, this approach reduces energy expenditure by 30-90%. These initial experiences give rise to our vision of LLM-based meta-compilers as a tool for students to transform high-level algorithms into efficient, hardware-specific implementations. Complementing this tooling, we will incorporate systems thinking concepts into the learning module so that students can reason both locally and globally about the effects of energy optimizations.

==> abstract-long.tex <==
\begin{abstract}
\emph{Background:} The increasing carbon footprint associated with rising energy consumption of data centers is becoming a growing concern for social and environmental well-being.
Despite the mounting concerns, energy-efficient programming techniques remain largely absent in software engineering and systems texts used in undergraduate education.
\emph{Aims:} We hope to address this gap by exploring ways to integrate energy-efficient computing methods into STEM education with the aid of large language models.
With the aid of LLMs, many algorithms can be customized to target specific architectures, which often provide energy-efficient instructions that are not well-understood by anyone other than experts in programming languages and computer systems/architecture.
%\JD{It would be nice to talk here about more systems level concerns and bring in the systems thinking angle.}
\GKT{I grabbed (and revised for abstract) some language from our paper to address Jamie's comment.}
We specifically focus on incorporating systems thinking to address challenges that demand high-level, holistic solutions.
\emph{Methods:} Our initial efforts have been focused on using LLMs to generate energy-efficient versions of basic linear algorithms on ARM64 and AMD64 architectures.
We leverage LLMs not only to create these energy-efficient versions but also to provide proper unit tests, a key component of reliable software engineering.
We then perform energy measurements.
All solutions are maintained in a prompt catalog and maintained as a collection of curricular materials using the Sphinx open source documentation tool (from the Python community).
\emph{Results:}
%\GKT{We need to put a proper number, not X\%. We should be able to get this from the proposal.}
Early results show that LLM can help reduce energy expenditure by 30-90\% for certain linear algebra operations on a variety of computer architectures, following the standard model that reducing processing time reduces energy consumption~\cite{barrosoCaseEnergyProportionalComputing2007}.
Beyond the performance gains, we have initial evidence to support that curricular materials employing systems thinking can be a valuable living resource for improving the efficacy of systems teaching and improving student engagement.
An expanded paper will generalize the results beyond our initial linear algebra examples and include dissemination via our website and permanent archival at ArXiv, Zenodo, and GitHub.
\end{abstract}

